DIFFNAT: Improving Diffusion Image Quality Using Natural Image Statistics

Diffusion models have advanced generative AI significantly in terms of editing and creating naturalistic images. However, efficiently improving generated image quality is still of paramount interest. In this context, we propose a generic "naturalness" preserving loss function, viz., kurtosis concentration (KC) loss, which can be readily applied to any standard diffusion model pipeline to elevate the image quality. Our motivation stems from the projected kurtosis concentration property of natural images, which states that natural images have nearly constant kurtosis values across different band-pass versions of the image. To retain the "naturalness" of the generated images, we enforce reducing the gap between the highest and lowest kurtosis values across the band-pass versions (e.g., Discrete Wavelet Transform (DWT)) of images. Note that our approach does not require any additional guidance like classifier or classifier-free guidance to improve the image quality. We validate the proposed approach for three diverse tasks, viz., (1) personalized few-shot finetuning using text guidance, (2) unconditional image generation, and (3) image super-resolution. Integrating the proposed KC loss has improved the perceptual quality across all these tasks in terms of both FID, MUSIQ score, and user evaluation.

==> motivation.tex <==
\section{Motivation}
In this section, we conduct an experiment to compare the image quality and noise of the natural images with that of generated images from DreamBooth and our method.
Although diffusion models generate high quality visual images, we want to investigate whether they have differences based on image statistics compared to natural images.
For image quality, we use the well-known metric MUSIQ~\cite{ke2021musiq}, which measures the image quality in multi-scale with varying size and aspect ratio of the image. 

\begin{wraptable}{r}{0.40\textwidth}
% \begin{table}[!h]
  %\scriptsize
  \small
  \centering
  %\scalebox{0.95}{
  \caption{Comparison of MUSIQ image quality metric and its relation to image noise}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{lccc}
  \toprule
  {\bf Method} & {\bf MUSIQ score $\uparrow$} & {\bf Noise $\sigma^2$ $\downarrow$} \\ 
  \midrule
  {DreamBooth~\cite{ruiz2022dreambooth}} & {68.319} & {0.382} \\
  {DreamBooth~\cite{ruiz2022dreambooth} + KC loss} & {68.319} & {0.372} \\
  {Custom diffusion~\cite{kumari2022multi}} & {70.15} & {0.351} \\
  {Custom diffusion~\cite{kumari2022multi} + KC loss} & {72.22} & {0.33} \\
  {Natural images} & {\bf 78.50} & {\bf $3 \times 10^{-47}$ ({$\sim$ 0})} \\  	  
  \bottomrule
  \end{tabular}}
  \label{table:sig_musiq_compare}
 % \end{table}
\end{wraptable}

  
To estimate the noise standard deviation of an image, we adopt the RiskShrink~\cite{donoho1992ideal} method, which is based on the absolute deviation of the wavelet detail coefficients. This well-known method assumes the noise follows a Gaussian distribution and estimates the noise standard deviation parameter. More details are provided in the supplementary material. To estimate this metric, we use the \texttt{skimage.estimate\_sigma} function from the skimage library~\cite{van2014scikit}, which provides us a reliable estimation of the noise statistics. 

In Tab.~\ref{table:sig_musiq_compare}, we compare both the average image quality metric MUSIQ and noise estimation metric. We observe that natural images have higher MUSIQ score and low noise standard deviation. 
Strikingly, the noise standard deviation alone can distinguish between the natural images and DreamBooth generated images, despite of the fact that DreamBooth generated images looks quite natural.
This observation motivates us to minimize the noise variance in the diffusion model generated image to make the generated images more natural. To minimize the noise variance, we rely on the kurtosis acorss the bandpass version of the image due to the kurtosis concentration property and propose a framework, viz., DiffNat to improve image quality in diffusion generated image. Our method indeed reduce the noise variance compared to DreamBooth as shown in Tab.~\ref{table:sig_musiq_compare}.

